Generalized mean shift with triangular kernel profile

The mean shift algorithm is a popular way to find modes of some probability density functions taking a specific kernel-based shape, used for clustering or visual tracking. Since its introduction, it underwent several practical improvements and generalizations, as well as deep theoretical analysis mainly focused on its convergence properties. In spite of encouraging results, this question has not received a clear general answer yet. In this paper we focus on a specific class of kernels, adapted in particular to the distributions clustering applications which motivated this work. We show that a novel Mean Shift variant adapted to them can be derived, and proved to converge after a finite number of iterations. In order to situate this new class of methods in the general picture of the Mean Shift theory, we alo give a synthetic exposure of existing results of this field.

==> 3-Median_Shift.tex <==

\section{Median shift}
\label{sect::Median_Shift}

The applicative need which initiated the present work is histogram clustering, for which the Wasserstein distance defined in Section \ref{sect::WMS} by Equation \eqref{eq::wasserstein_metric} is much more meaningful than the Euclidean distance. We will see that working with the Wasserstein metric can be reduced to working with the $L_1$-norm, so we first analyze this case in Section \ref{sect::Mean_Shift_L1}.


\subsection{Adapting Mean shift to $L_1$ norm}
\label{sect::Mean_Shift_L1}
Replacing $L_2$-norm with $L_1$-norm in Equation \eqref{eq::ker_density} and using the triangular kernel (defined by $K(u) = \max(1-u,0)$) the p.d.f. under study becomes:
$$
f(x) = \sum_{i \in C(x)} \left( 1- \norm{x-x_i}_1 \right),
$$
where $\norm{\cdot}_1$ denotes the $L_1$-norm in $\RR^q$ and $C(x) = \{ i \in [1,N], \norm{x-x_i}_1 < 1 \}$ is the set of  indices $i$ for which we have $K(\norm{x-x_i}_1) \not= 0$. The triangular kernel $K(\cdot)$ used here is not differentiable at $1$, but any value taken in the interval $[-1,0]$ is a sub-derivative of $K(\cdot)$ at 1. We choose $0$ (other choices are possible) to build the function $g(\cdot)$ of Algorithm \ref{algo::Mean_Shift_generalized}, which gives $g(u)=1$ for $u<1$ and $g(u)=0$ for $u\geq 1$. The bounding functions $\hat{f}_n(\cdot)$ appearing in Algorithm \ref{algo::Mean_Shift_generalized} are then defined by:
$$
\hat{f}_n(x) = \sum_{i\in C(\hat{x}_n)} \left( 1- \norm{x-x_i}_1 \right)
$$
Maximizing $\hat{f}_n(\cdot)$ is equivalent to minimizing $\sum_{i\in C(\hat{x}_n)} \norm{x-x_i}_1$ over $x$, which is achieved by the coordinate-by-coordinate median of the set $\{ x_i, i\in C(\hat{x}_n) \}$. This immediately leads to Algorithm \ref{algo::MS_L1}.
%
%%%%%%%%%%%% ALGO MEDIAN SHIFT %%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}
\caption{Median shift}
\label{algo::MS_L1}
\begin{algorithmic}
\STATE Choose an initial seed $\hat{x}_0$.
\FOR{$n=1:$ Max\_Iteration}
\STATE 
\begin{equation}
%\label{eq::rrr}
\hat{x}_{n+1} = \text{Median} \{ x_i ,  \left| \left| x_i - \hat{z}_n \right| \right|_ 1 <1 \}.
\end{equation}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
%
Proposition \ref{prop::growth_generalized} ensures the value of $f(\hat{x}_n)$ (with $\hat{x}_n$ returned by Algorithm \ref{algo::MS_L1}) increases at each iteration of Algorithm \ref{algo::MS_L1}. But the $L_1$ case is especially convenient and we can also show the convergence of $\hat{x}_n$:

\begin{prop}
\label{prop::L_1_convergence}
The sequence of mode estimates returned by Algorithm \ref{algo::MS_L1} is convergent (more specifically it is stationnary) for any initialization.
\end{prop}
\begin{proof}
To help understanding the proof, we divide it into three steps:
\begin{description}
\item[step 1:] There exist $p \in \NN$ ensuring the property $\forall n\geq p, f(\hat{x}_n) \geq f(\hat{x}_p)$ (i.e. $f(\hat{x}_n)$ is stationary).
\item[step 2:] From rank $n=p$ (with $p$ defined in step 1), the set-valued sequence $C(\hat{x}_n)$ is decreasing for the inclusion.
\item[step 3:] The sequence $\hat{x}_n$ is stationary.
\end{description}
The steps 1, 2 and 3 are shown as follows:
\begin{description}
\item[Proof of step 1:] Each $\hat{x}_n$ for $n \geq 1$ is the median of a subset of the data point cloud $(x_1,\dots,x_N)$. As there is only a finite number of such subsets, $\hat{x}_n$ can only take a finite number of values. Consequently, this is also the case for its image $f(\hat{x}_n)$. As $f(\hat{x}_n)$ is moreover growing (Proposition \ref{prop::growth_generalized}), we can conclude it is stationary, i.e., there exists a rank $p \in \NN$ ensuring $f(\hat{x}_n)=f(\hat{x}_p)$ for any $n \geq p$.
\item[Proof of step 2:] For each $n \geq p$, we decompose $f(\hat{x}_{n+1})$ as follows:
\begin{align*}
f(\hat{x}_{n+1}) = & \sum_{i=1}^N K(||\hat{x}_{n+1}-x_i||_1) = \sum_{i \in C(\hat{x}_{n+1})} \left( 1-||\hat{x}_{n+1}-x_i||_1 \right) 
 =  A+B-D,
\end{align*}
with $A$,$B$,$D$ defined as:
\begin{align*}
A & = \sum_{i \in C(\hat{x}_n)} \left( 1-||\hat{x}_{n+1}-x_i||_1 \right), \\
B & = \sum_{i \in C(\hat{x}_{n+1}) \backslash C(\hat{x}_n)} \left( 1-||\hat{x}_{n+1}-x_i||_1 \right), \\
D & = \sum_{i \in C(\hat{x}_n) \backslash C(\hat{x}_{n+1})} \left( 1-||\hat{x}_{n+1}-x_i||_1 \right).
\end{align*}
Let us study these three quantities.
\begin{itemize}
\item Following Equation \eqref{eq::iterate} we have $A \geqslant \sum_{i \in C(\hat{x}_n)} \left( 1-||x-x_i||_1 \right)$ for any $x \in \RR^q$. In particular, $A \geqslant \sum_{i \in C(\hat{x}_n)} \left( 1-||\hat{x}_n-x_i||_1 \right)$, i.e., $A \geqslant f(\hat{x}_n)$.
\item All indices $i$ of the set $C(\hat{x}_{n+1}) \backslash C(\hat{x}_n)$ belonging to  $C(\hat{x}_{n+1})$, they ensure $(1-\norm{\hat{x}_{n+1}-x_i}_1) >0$. Thus, $B$ is a sum of (strictly) positive terms. In particular, we have $B \geq 0$.
\item All indices $i \in C(\hat{x}_n) \backslash C(\hat{x}_{n+1})$ being outside $C(\hat{x}_{n+1})$, they ensure $(1-\norm{\hat{x}_{n+1}-x_i}_1)  \leq 0$. Thus, $D$ is a sum of non-positive terms. In particular, we have $D \leq 0$.
\end{itemize}
The inequality $A \geqslant f(\hat{x}_n)$ gives $f(\hat{x}_{n+1}) - f(\hat{x}_n) \geq B+ (-D)$. As we chose $n \geq p$, step 1 ensures $f(\hat{x}_{n+1}) - f(\hat{x}_n) = 0$ and we obtain $ 0 \geq B+ (-D)$. The two terms of the sum $B+(-D)$ being non-negative, the inequality $ 0 \geq B+ (-D)$ implies $B=0$ and $D=0$. The terms appearing in the sum defining $B$ being strictly positive, the number of terms is necessarily zero, i.e., we have $C(\hat{x}_{n+1}) \backslash C(\hat{x}_n) = \emptyset$, i.e. $C(\hat{x}_{n+1}) \subset C(\hat{x}_n)$. The reasoning holds for any $n \geq p$, meaning the set-valued sequence $C(\hat{x}_n)$ is decreasing (for the set inclusion) after rank $n=p$.
\item[Proof of step 3:]
The set-valued sequence $C(\hat{x}_n)$ is decreasing for the set inclusion order after rank $p$ (see step 2). Moreover, $C(\hat{x}_n)$ is always a subset of the point cloud so it cannot take more than $2^N$ different values (the number of subsets of the point cloud). As a consequence, again, the sequence $(C(\hat{x}_n))_{n \geq 0}$ is stationary. Thus, its median $\hat{x}_{n+1}$ is also stationary.
\end{description}
\end{proof}

\begin{rem}
The property shown in step 2 in the proof of Proposition \ref{prop::L_1_convergence} may look convoluted as in most cases, the set $C(\hat{x}_n)$ stops changing as soon as $f(\hat{x}_n)$ reaches its final value. But here, $C(\hat{x}_n)$ being decreasing for the inclusion cannot be replaced with $C(\hat{x}_n)$ being constant. Indeed, adapting the proof would require the number $D$ to be a sum of strictly negative (instead of non-positive) terms, which is not true due to the possibility for some points of the dataset to end up on the boundary of $C(\hat{x}_n)$. The weaker statement of step 2 allows handling this situation.
\end{rem}

\subsection{Adapting Mean shift to the Wasserstein metric}
\label{sect::WMS}

The Wasserstein metric, also called the Earth Moving Distance, is a distance function between probability distributions on a set $U$. It is defined for a given $p\in \NN$ and two probability measures $\mu$ and $\nu$ on $U$ as:
\begin{equation}
W_{p}(\mu,\nu) = \inf_{\gamma \in \Gamma(\mu,\nu)} \int_{U \times U} d(x,y)^p d\gamma(x,y),
\end{equation}
where $\Gamma (\mu,\nu)$ is the collection of all probability distributions on $U \times U$ with marginals $\mu$ and $\nu$ over the first and second variable respectively.

We focus here on the specific case where $U$ is a finite set of cardinal $q$, $d(\cdot,\cdot)$ is the $L_1$-norm and $p=1$. Under these hypotheses, $\mu$ and $\nu$ can be encoded through their histograms $M$ and $N \in \RR^q$ and the Wasserstein metric can be shown to take the simpler form below:
\begin{equation}
\label{eq::wasserstein_metric}
W_{1}(M,N) = ||CH(M)-CH(N)||_{L1} = ||CH(M-N)||_{L1},
\end{equation}
where $CH(x)$ denotes the cumulative sum of a vector $ x=(x^1,x^2,\dots,x^q) \in \RR^q $:
$$\left[CH(x)\right]^k = \sum_{j=1}^k x^j.$$
This function is easily inverted:
$$ \left[ CH^{-1}(z) \right]^k = \Big \{ \begin{matrix}
(z^k-z^{k-1}) & \text{for} & k >1, \\
z^1 & \text{for} & k =1.
\end{matrix} $$
\begin{rem}
The points of the data set $\RR^q$ being denoted with a subscript ($i$ or $n$) in this paper, their coordinates will be denoted with a superscript to avoid confusion.
\end{rem}
Proposition \ref{prop::WMS_optimization} shows that the general algorithm \ref{algo::Mean_Shift_generalized} is still tractable when used with the Wasserstein metric. This result is expected given the relation between Wasserstein metric and $L_1$-norm (Equation \eqref{eq::wasserstein_metric}). Yet, Lemma \ref{lem::histo} below is necessary to first settle the only subtlety arising in the proof of Proposition \ref{prop::WMS_optimization}.
\begin{lem}
\label{lem::histo}
Let $(z_1,z_2,\dots,z_P)$ be a set of $P$ cumulated histograms of size $q$. Then their term-by-term median $\tilde{z}$ is also the cumulative histogram of a discrete distribution $x \in \RR^q$.
\end{lem}
\begin{proof}
To be a cumulative histogram, the median $\tilde{z}$ has to verify:
\begin{enumerate}
\item $\tilde{z}^1 \geq 0$, \label{lem::histo1}
\item $\forall k \in [1,q-1],\tilde{z}^{k+1}\geq \tilde{z}^k$, \label{lem::histo2}
\item $\tilde{z}^q =1$. \label{lem::histo3}
\end{enumerate}
Properties \eqref{lem::histo1} and \eqref{lem::histo3} are immediate (the median of non-negative numbers is non-negative and the median of $q$ times the number 1 is still 1). Property \eqref{lem::histo2} is shown as follows.

For each $k \in [1:q]$ we denote by $I^k_+ = \{ i \in [1,P], z^k_i \geq \tilde{z}^k \}$ the set of indices $i$ for which $z_i^k$ is above the median computed on coordinate $k$. By definition of the median we have:
$$
Card(I^k_+) \geq E((P+1)/2)
$$
where E denotes the integer part. As each $z_{j}$ is a cumulative histogram, we have:
\begin{equation}
\label{eq6}
\forall j \in c^{k}_{+}\, z^k_{j} \leq z^{k+1}_{j}
\end{equation}
\ref{eq5} and \ref{eq6} imply:
\begin{equation}
\label{eq8}
\forall j \in c^{k}_{+}\, \hat z^{k} \leq z^{k+1}_{j}
\end{equation}
following \ref{eq7}, the equation \ref{eq8} implies:
\begin{equation}
\label{eq9}
Card(\{j \mid \tilde z_{k} \leq z_{j}^{k+1}\}) \geq Card(c^{k}_{+}) \geq E((n+1)/2)
\end{equation}
which means we can find at least $E((n+1)/2)$ $z^{k+1}_j$ that are greater than $\hat z^k$ amongst the $z^{k+1}_{j}$. Thus this is also verified by their median. This implies: 
\begin{equation*}
\hat z^{k} \leq \hat z^{k+1}
\end{equation*}

\end{proof}

 of Proposition \ref{prop::WMS_optimization}

\begin{prop}
\label{prop::WMS_optimization}
If Algorithm \ref{algo::Mean_Shift_generalized} is used with $d=W_1$ (see Equation \eqref{eq::wasserstein_metric}), $p=1$ and triangular kernel, then the optimization step is solved by: 
\begin{equation}
\label{eq::WMS_CD}
\hat{x}_{n+1} = CH^{-1} ( \text{Median} \{  CH(x_i), \norm{ CH(\hat{x}_n-x_i)}_1  <1 \} ).
\end{equation}
\end{prop}
\begin{proof}
For a given $n \in \NN$ we consider the cumulated histograms of the involved variables: $\hat{z}_n = CH(\hat{x}_n)$, $z_1=CH(x_1), z_2 = CH(x_2), \dots, z_n = CH(x_n)$. Then, the optimization step of Algorithm can be \ref{algo::Mean_Shift_generalized} performed directly on the cumulated histograms. We obtain the following optimization problem:
\begin{equation}
\label{eq::constrained}
\hat{z}_{n+1} = \min_z \sum_{i \in C_i} \norm{z-\hat{z}_i}_1, \text{ subject to } z \in CH(\RR^q).
\end{equation}
As before, the sets $C_i$ are defined as $C_i = \{ z \in \RR^q, \norm{z-\hat{z}_i}_1<1 \} $
The constraint $z \in CH(\RR^q)$ means that the returned optimum $\hat{z}_{n+1}$ has to be a cumulative histogram. This is equivalent to the combination of the two constraints \ref{prop::ck} and \ref{prop::sum1} below:
\begin{enumerate}
\item $ \forall k =1,\dots,q-1  \quad  \hat{z}_{k+1} \geq \hat{z}_k.$ \label{prop::ck}
\item $ \hat{z}_q = 1.$ \label{prop::sum1}
\end{enumerate}
The solution of the unconstrained counterpart of \eqref{eq::constrained} is well known: it is given by the coordinate-by-coordinate median of the set of vectors $z_1,\dots,z_N$. To ensure that it also solves \eqref{eq::constrained} we have to check that the median still verifies the constraints.
\paragraph{Constrainst \ref{prop::ck}:}
We consider a set $\{z_{1},\dots,z_{N}\}$ of cumulative histograms and its term-by-term median $\hat{z}$.
Let $c^{k}_{+}$ be the set of indices $j$ such that :
\begin{equation}
\label{eq5}
\hat z^k \leq z^k_{j}
\end{equation}
by definition of the median we have:
\begin{equation}
\label{eq7}
Card(c^{k}_{+})\geq E((n+1)/2)
\end{equation}
where E denotes the integer part.
As each $z_{j}$ is a cumulative histogram, we have:
\begin{equation}
\label{eq6}
\forall j \in c^{k}_{+}\, z^k_{j} \leq z^{k+1}_{j}
\end{equation}
\ref{eq5} and \ref{eq6} imply:
\begin{equation}
\label{eq8}
\forall j \in c^{k}_{+}\, \hat z^{k} \leq z^{k+1}_{j}
\end{equation}
following \ref{eq7}, the equation \ref{eq8} implies:
\begin{equation}
\label{eq9}
Card(\{j \mid \tilde z_{k} \leq z_{j}^{k+1}\}) \geq Card(c^{k}_{+}) \geq E((n+1)/2)
\end{equation}
which means we can find at least $E((n+1)/2)$ $z^{k+1}_j$ that are greater than $\hat z^k$ amongst the $z^{k+1}_{j}$. Thus this is also verified by their median. This implies: 
\begin{equation*}
\hat z^{k} \leq \hat z^{k+1}
\end{equation*}

\paragraph{Constrainst \ref{prop::sum1}:}
As all the $z_{i}$ are cumulative histogram, we have:
\begin{equation*}
\forall i  \quad z^q_{i}=1
\qquad
 z^1_{i}=0
\end{equation*}
which implies by definition of $\hat{z}$:
\begin{equation*}
\hat{z}^q=1
\qquad
\hat{z}^1=0.
\end{equation*}
%If $k$ is the triangular kernel, its derivative $k'$ is defined as $k'(u)=-1\!\!1_{u<1}$. The optimization step in Algorithm \ref{algo::Mean_Shift_generalized} is then $\hat{x}_{n+1} = \text{argmin} \sum_i || CD(x) - CD(x_i) ||_1 1\!\!1_{|| CD(\hat{x}_n) - CD(x_i) ||_1}$. we see the argument $x$ of the minimization appears only through its image $CD(x)$. Thus, the problem can be reformulated as $CD(x) = $
\end{proof}
As $x$ is easily retrieved from $CH(x)$, Proposition \ref{prop::WMS_optimization} provides a closed-form formula for the optimization problem appearing in Algorithm \ref{algo::Mean_Shift_generalized}. It makes the adaptation of Mean Shift tractable in practice, but also suggests directly working on the cumulative histograms. This idea ends in Algorithm \ref{algo::WMS} (Wasserstein median shift).
\begin{algorithm}
\caption{Wasserstein median shift}
\label{algo::WMS}
\begin{algorithmic}
\STATE Compute $z_i =CH(x_i)$ for each $i$.
\STATE Choose an initial seed $\hat{z}_0$.
\FOR{$n=1:$ Max\_Iteration}
\STATE
\begin{equation}
\hat{z}_{n+1} = \text{Median} \{ z_i ,  \left| \left| z_i - \hat{z}_n \right| \right|_ 1 <1 \}.
\end{equation}
\STATE $\hat{x}_n = CH^{-1}(\hat{z}_n)$.
\ENDFOR
\end{algorithmic}
\end{algorithm}
Following Proposition \ref{prop::WMS_convergence}, the obtained estimate $\hat{x}_n$ is again stationary.

Section \ref{sect::Results} will now illustrate the benefits of Algorithm \ref{algo::WMS} on both synthetic and real data.


==> README <==
LaTeX package 'ifoddpage'
~~~~~~~~~~~~~~~~~~~~~~~~
Copyright (c) 2011 by Martin Scharrer <martin@scharrer-online.de>
WWW: http://latex.scharrer-online.de/
CTAN: http://www.ctan.org/pkg/ifoddpage
Code repository: https://bitbucket.org/martin_scharrer/ifoddpage

This LaTeX package provides a \ifoddpage conditional to determine if the current page is odd or even.
The macro \checkoddpage must be used direct before to check the page number using a label.
Two compiler runs are therefore required to achieve correct results.
In addition the conditional \ifoddpageoronside is provided which is also true in oneside mode where 
all pages use the odd page layout.

This package got inspired from the 'changepage' package which provides (and uses) the same macros (\checkoddpage and
\ifoddpage) for its main function of changing the page design mid-way in the document.  Both packages can be used
together, but the 'ifoddpage' should be loaded last in this case, otherwise the \ifoddpageoroneside conditional will
stop working.



==> fp.tex <==
%load the fp-package for TeX
\chardef\FPcatamp=\the\catcode`\@
\catcode`@=11

\def\NeedsTeXFormat#1{}
\def\ProvidesPackage#1[#2]{}
\def\DeclareOption#1#2{}
\let\ProcessOptions\relax

%the for-loop of latex2e
\def\@nnil{\@nil}
\def\@empty{}
\def\@fornoop#1\@@#2#3{}
 
\def\@for#1:=#2\do#3{\edef\@fortmp{#2}\ifx\@fortmp\@empty \else
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}\fi}
 
\def\@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\@nnil \else
       #5\def#4{#2}\ifx #4\@nnil \else#5\@iforloop #3\@@#4{#5}\fi\fi}
 
\def\@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\@nnil
       \let\@nextwhile\@fornoop \else
      #4\relax\let\@nextwhile\@iforloop\fi\@nextwhile#2\@@#3{#4}}

\edef\FP@loadedfiles{fp.tex}

\def\FP@alreadyloaded#1{}
\def\FP@notyetloaded#1{
  \edef\FP@loadedfiles{\FP@loadedfiles,#1}
  \input #1.sty
}
\def\RequirePackage#1{%
  \let\FP@in@\FP@notyetloaded%
  \edef\@tempb{#1}%
  \@for\@tempa:=\FP@loadedfiles\do{%
    \ifx\@tempa\@tempb%
      \let\FP@in@\FP@alreadyloaded%
    \fi%
  }%
  \FP@in@{#1}%
} 

\def\loop#1\repeat{\def\iterate{#1\relax\expandafter\iterate\fi}%
  \iterate \let\iterate\relax}
\let\repeat=\fi

\RequirePackage{fp}

\catcode`\@=\FPcatamp

